To Ba or not to Ba: Enrichment in s-process elements in binary systems with WD companions of various masses

The enrichment in s-process elements of barium stars is known to be due to pollution by mass transfer from a companion formerly on the thermally-pulsing asymptotic giant branch (AGB), now a carbon-oxygen white-dwarf (WD). This paper investigates the relationship between the s-process enrichment in the barium star and the mass of its WD companion. It is expected that helium WDs, which have masses smaller than about 0.5 Msun and never reached the AGB phase, should not pollute with s-process elements their giant companion, which should thus never turn into a barium star. Spectra with a resolution of R ~ 86000 were obtained with the HERMES spectrograph on the 1.2-m Mercator telescope for a sample of 11 binary systems involving WD companions of various masses. We use standard 1D LTE MARCS model atmospheres coupled with the Turbospectrum radiative-transfer code to derive the atmospheric parameters using equivalent widths of FeI and Fe II lines. The abundances of s-process elements for the entire sample of 11 binary stars were derived homogeneously. The sample encompasses all levels of overabundances: from solar [s/Fe]=0 to 1.5 dex in the 2 binary systems with S-star primaries (for which dedicated MARCS model atmospheres were used). The primary components of binary systems with a WD more massive than 0.5 Msun are enriched in s-process elements. We also found a trend of increasing [s/Fe] with [C/Fe] or [(C+N)/Fe]. Our results conform to the expectation that binary systems with WD companions less massive than 0.5 Msun do not host barium stars.

==> abundances.tex <==
\begin{tabular}{lcrrcrl}
  \multicolumn{3}{l}{IP Eri} \\
  \hline 
    X  & A(X) & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\
  C  & 8.62 & $ 0.23$ & $ 0.14$ & 0.10 &  5 & \ion{C}{i} lines \\
  C  & 8.34 & $-0.05$ & $-0.14$ & 0.16 & 18 & C$_2$ lines \\
  N  & 7.64 & $-0.14$ & $-0.23$ & 0.06 & 96 &\ion{N}{i} + CN lines \\ 
  O  & 8.89 & $ 0.23$ & $ 0.14$ &  -   &  1 & [\ion{O}{i}] $\lambda$630.03 \\
  \\ 
  Fe I  & 7.56 & $0.11$ &         &  $0.13$ &  87 \\
  Fe II & 7.53 & $0.08$ &         &  $0.12$ &  16 \\
  \\
  Sr I  & 3.10 & $ 0.18$ & $ 0.09$ & 0.04 &   3 &    \\
  Y  I  & 2.33 & $ 0.12$ & $ 0.03$ & 0.05 &   2 & $\lambda$619.17, $\lambda$643.50 \\
  Y II  & 1.94 & $ 0.27$ & $ 0.18$ & 0.11 &   5 &  \\
  Zr I  & 2.89 & $ 0.31$ & $ 0.22$ & 0.18 &   4 & \\
  Zr II & 2.82 & $ 0.24$ & $ 0.15$ & 0.01 &   2 & $\lambda$444.30, $\lambda$535.01 \\
  \\
  Ba II & 2.44 & $ 0.27$ & $ 0.18$ & 0.04 &   4 & \\
  La II & 1.17 & $ 0.04$ & $-0.05$ & 0.14 &  10 & \\
  Ce II & 1.57 & $-0.13$ & $-0.22$ & 0.08 &   4 & \\
  Nd II & 1.50 & $+0.05$ & $-0.04$ & 0.12 &   8 & \\
  \\
   \multicolumn{3}{l}{$\zeta$ Cap} \\
  \hline 
    X  & A(X) & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\ 
  C     &  8.60  & $ 0.21$ & $ 0.29$ & 0.04 &   4 & \ion{C}{i} lines \\
  C     &  8.42  & $ 0.03$ & $ 0.11$ & 0.05 &  16 & C$_2$ lines \\
%  C     &  8.48  & $ 0.09$ & $ 0.17$ & 0.17 &  36 & CH bands \\
%  N I   &  8.05  & $ 0.27$ & $ 0.35$ & 0.10 &   9 & atomic lines \\
  N     &  8.08  & $ 0.30$ & $ 0.38$ & 0.07 &  85 & \ion{N}{i} + CN lines \\
  O    &   8.70  & $ 0.04$ & $ 0.12$ & 0.08 & 2 & \ion{O}{i} lines \\
%  O I   &  9.10  & $ 0.44$ & $ 0.52$ & 0.28 &   7 & from atomic lines \\
  \\  
%  Na    &  6.34  & $ 0.17$ & $ 0.25$ & 0.23 &   (9) & without doublets \\
%  Mg    &  7.58  & $ 0.05$ & $ 0.13$ & 0.15 &  (14) & \\
%  Al    &  6.42  & $ 0.05$ & $ 0.13$ & 0.08 &   (7) & \\
%  Si    &  7.48  & $-0.03$ & $ 0.05$ & 0.20 &  (22) & \\ 
  \\
Sr I & $3.86$ & & & $0.06$ & 2 \\
%  Sr I  &  3.89  & $ 0.97$ & $ 1.05$ & 0.14 &   4 & \\
%  Y I   &  3.33  & $ 1.12$ & $ 1.20$ &    - &   1 & $\lambda$643.50 \\
%  Y II  &  3.49  & $ 1.28$ & $ 1.36$ & 0.28 &   9 & \\
%  Zr I  &  3.58  & $ 1.00$ & $ 1.08$ & 0.24 &   6 & \\  
%  Zr II &  3.94  & $ 1.36$ & $ 1.44$ & 0.11 &   4 & \\ 
%  \\
%  Ba I  &  3.37  & $ 1.20$ & $ 1.28$ &    - &   1 & $\lambda$705.99 \\
%  Ba II &  3.84  & $ 1.67$ & $ 1.75$ & 0.36 &   5 & \\
%  La II &  2.26  & $ 1.13$ & $ 1.21$ & 0.27 &  16 & \\
%  Ce II &  2.53  & $ 0.83$ & $ 0.91$ & 0.23 &  13 & \\ 
%  \\
%  Pb I  &  2.09  & $ 0.09$ & $ 0.17$ & 0.30 &   1 & $\lambda$405.78 \\
  \\
    \multicolumn{3}{l}{$\zeta$ Cyg} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\  
  C    & $8.43$ & $ 0.04$ & $ 0.07$ & 0.13 &  4 & \ion{C}{i} lines \\
  C    & $8.14$ & $-0.25$ & $-0.22$ & 0.13 & 15 & C$_2$ lines \\
  N    & $7.86$ & $ 0.08$ & $ 0.11$ & 0.05 & 94 & \ion{N}{i} + CN lines\\
  O    & $8.79$ & $ 0.13$ & $ 0.16$ & 0.06 & 2 &  \ion{O}{i} lines \\
  \\
    \multicolumn{3}{l}{63 Eri} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\  
  C    & $8.10$ & $-0.29$ & $-0.11$ & 0.21 &  3 & \ion{C}{i} lines\\
  C    & $8.09$ & $-0.30$ & $-0.12$ & 0.18 & 13 & C$_2$ lines     \\
  N    & $7.71$ & $-0.07$ & $ 0.25$ & 0.05 & 50 & \ion{N}{i} + CN lines\\
  O    & $8.79$ & $ 0.13$ & $ 0.31$ & 0.04 & 6 &  \ion{O}{i} lines \\
  \\
  \\
    \multicolumn{3}{l}{56 Peg} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\  
  C   & 8.13 & $-0.26$ & $ 0.19$ & 0.02  &  4 & \ion{C}{i} lines\\
  C   & 7.95 & $-0.44$ & $ 0.01$ & 0.23  & 13 & C$_2$ lines     \\
  N   & 7.16 & $-0.62$ & $-0.17$ & 0.07  & 82 & \ion{N}{i} + CN lines\\
  O   & 8.33 & $-0.33$ & $ 0.12$ &  -    & 1 & [\ion{O}{i}] $\lambda$630.03 \\
  \\
    \multicolumn{3}{l}{14 Aur C} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\  
  C   & 8.47 & $ 0.08$ & $0.19$ & 0.24 & 2 & \ion{C}{i} lines\\
  C   & 8.50 & $ 0.11$ & $0.22$ & 0.03 & 3 & C$_2$ lines     \\
  N   & 7.92 & $ 0.14$ & $0.25$ & 0.13 & 4 & CN lines\\
  O   & 8.61 & $-0.05$ & $0.16$ &  -   & 1 & \ion{O}{i} 615.68\\
  \\
    \multicolumn{3}{l}{HR5692} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\  
  C  & 8.41 & $ 0.02$ & $ 0.10$ & 0.02 &  5 &  \ion{C}{i} lines\\
  C  & 8.05 & $-0.34$ & $-0.24$ & 0.10 & 10 &  C$_2$ lines     \\  
  N  & 7.54 & $-0.24$ & $-0.16$ & 0.08 & 90 & \ion{N}{i} + CN lines\\
  O  & 8.78 & $ 0.12$ & $ 0.20$ & -    &  1 & [\ion{O}{i}] $\lambda$630.03 \\
  \\
    \multicolumn{3}{l}{DR Dra} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\  
  C  & 8.26 & $-0.13$ & $ 0.01$ & 0.23 &  3 &  \ion{C}{i} lines \\
  C  & 8.02 & $-0.37$ & $-0.23$ & 0.07 &  8 &  C$_2$ lines      \\
  N  & 7.43 & $-0.35$ & $-0.21$ & 0.09 & 82 & \ion{N}{i} + CN lines\\
  O  & 8.67 & $+0.01$ & $ 0.15$ & -    &  1 & [\ion{O}{i}] $\lambda$630.03 \\
\\
    \multicolumn{3}{l}{V1261 Ori} \\
  \hline 
    X   & A(X)   & [X/H] & [X/Fe] & $\sigma_\mathrm{stat}$ &  N & comments\\
  \hline \\
  C & 8.40 & $ 0.00$ & $ 0.67$ & 0.14 & & \citet{Smith1990} \\
  N & 8.06 & $ 0.28$ & $ 0.94$ & 0.11 & & \citet{Smith1990} \\
  O & 8.80 & $ 0.14$ & $ 0.80$ & 0.08 & & \citet{Smith1990} \\
   \hline
 \end{tabular}
